When the Cheapest Feasible Router Fails: Auditing Deployment Commitments in Cost-Aware LLM Routing

Cost-aware LLM routing often selects the cheapest policy meeting empirical risk and coverage constraints. Yet a router that passes an audit can violate its fixed service contract on new requests, even when candidate policies are constructed independently. We study this deployment-commitment decision with disjoint construction, audit, and test samples. Across 19 RouterBench task families, the cheapest audit-feasible router deploys in 91.82% of opportunities but violates the held-out contract in 32.22% of deployments. We introduce Menu-Aware Routing Commitment (MARC), which qualifies policies using audit evidence and a serving-cost tolerance to retain the apparent winner, deploy a supported alternative, or defer. Its practical policywise variant (MARC-P) reduces observed conditional failure to 0.73% at 85.79% deployment, with higher serving cost; fixed-margin and formal risk-control procedures provide competitive alternatives. Nested audits show how added evidence changes deployable policy sets, and learned semantic routing exhibits the same commitment failure. These results establish deployment commitment as a distinct operational decision connecting router evaluation, service reliability, and inference cost.

==> tables/full_objective_grid.tex <==
\begin{table*}[!tp]\centering\scriptsize\setlength{\tabcolsep}{3pt}
\begin{tabular}{lrrrr|rrrr}\toprule
& \multicolumn{4}{c}{Mean-cost objective} & \multicolumn{4}{c}{Tail-cost objective} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
Procedure & Deploy & D\&F & Fail$\mid$D & Cost & Deploy & D\&F & Fail$\mid$D & Cost \\
\midrule
Audit winner & 91.82 & 29.52 & 32.14 & 0.00044 & 91.82 & 29.74 & 32.30 & 0.00075 \\
Independent gate & 62.98 & 12.43 & 21.28 & 0.00033 & 63.03 & 12.32 & 20.91 & 0.00055 \\
Fixed $.00$ & 91.82 & 29.17 & 31.78 & 0.00045 & 91.82 & 15.33 & 17.01 & 0.00083 \\
Fixed $.02$ & 89.89 & 18.33 & 20.46 & 0.00043 & 89.89 & 9.74 & 11.25 & 0.00076 \\
Fixed $.05$ & 87.72 & 7.94 & 9.36 & 0.00059 & 87.72 & 4.19 & 5.14 & 0.00098 \\
Fixed $.08$ & 86.93 & 3.33 & 4.08 & 0.00081 & 86.93 & 2.00 & 2.55 & 0.00124 \\
Fixed $.10$ & 86.32 & 1.73 & 2.12 & 0.00101 & 86.32 & 1.12 & 1.43 & 0.00145 \\
Fixed $.15$ & 82.74 & 0.37 & 0.47 & 0.00146 & 82.74 & 0.20 & 0.29 & 0.00191 \\
MARC-P $.00$ & 87.26 & 7.06 & 8.36 & 0.00055 & 87.26 & 2.96 & 3.81 & 0.00085 \\
MARC-P $.02$ & 86.71 & 2.92 & 3.46 & 0.00073 & 86.71 & 1.36 & 1.74 & 0.00112 \\
MARC-P $.05$ & 85.79 & 0.77 & 0.89 & 0.00107 & 85.79 & 0.48 & 0.57 & 0.00151 \\
MARC-S $.00$ & 75.48 & 0.37 & 0.47 & 0.00112 & 75.48 & 0.20 & 0.28 & 0.00155 \\
MARC-S $.02$ & 71.93 & 0.15 & 0.24 & 0.00113 & 71.93 & 0.11 & 0.18 & 0.00152 \\
MARC-S $.05$ & 68.03 & 0.00 & 0.00 & 0.00113 & 68.03 & 0.00 & 0.00 & 0.00148 \\
LTT-Bonf. & 78.38 & 0.09 & 0.12 & 0.00139 & 78.38 & 0.09 & 0.12 & 0.00184 \\
LTT-Holm & 78.38 & 0.09 & 0.12 & 0.00139 & 78.38 & 0.09 & 0.12 & 0.00183 \\
Pareto Testing & 84.41 & 0.53 & 0.66 & 0.00130 & 84.41 & 0.46 & 0.54 & 0.00171 \\
\bottomrule\end{tabular}\caption{RouterBench full method/buffer grid by optimization objective (dataset-equal rates; selected serving cost conditional on deployment; $\alpha=.10$).}\label{tab:full_objgrid}\end{table*}
